Personalized Predictions from Population Level Experiments: A Study on Alzheimer's Disease

The purpose of this article is to infer patient level outcomes from population level randomized control trials (RCTs). In this pursuit, we utilize the recently proposed synthetic nearest neighbors (SNN) estimator. At its core, SNN leverages information across patients to impute missing data associated with each patient of interest. We focus on two types of missing data: (i) unrecorded outcomes from discontinuing the assigned treatments and (ii) unobserved outcomes associated with unassigned treatments. Data imputation in the former powers and de-biases RCTs, while data imputation in the latter simulates "synthetic RCTs" to predict the outcomes for each patient under every treatment. The SNN estimator is interpretable, transparent, and causally justified under a broad class of missing data scenarios. Relative to several standard methods, we empirically find that SNN performs well for the above two applications using Phase 3 clinical trial data on patients with Alzheimer's Disease. Our findings directly suggest that SNN can tackle a current pain point within the clinical trial workflow on patient dropouts and serve as a new tool towards the development of precision medicine. Building on our insights, we discuss how SNN can further generalize to real-world applications.

==> content/abstract.tex <==
%
The focus of this work is to infer patient level clinical outcomes from {\color{orange} population level} randomized control trials (RCTs). 
%
Towards this, we utilize the recently proposed synthetic nearest neighbors (SNN) estimator, which leverages information across patients to impute missing data associated with each patient of interest. 
%
Two forms of missing data we focus on are:
%
(i) Unrecorded outcomes from patients discontinuing the assigned treatment---data imputation then enables accurate inferences from a RCT dataset that are no longer biased from such patient dropouts.
%
(ii) Unobserved outcomes associated with treatments a patient was not assigned---data imputation enables simulations of ``synthetic RCTs'', where outcomes for each patient under every treatment are predicted. 
%
Notably, the SNN~estimator is both {\color{orange} interpretable and transparent}, causally justified under a broad class of missing not at random data scenarios, and {\color{orange} operational under limited data constraints}. 
%
Using Phase 3 clinical trial data on patients with Alzheimer’s Disease, we illustrate SNN's utility for the above two applications.
%
{\color{orange} Add quantitative statement about SNN compared to baselines.}
%
In doing so, we tackle a current pain point within the clinical trial workflow of patient dropouts and provide a novel methodology towards the development of precision medicine. 
%
Lastly, we discuss how the SNN~estimator can generalize to post-clinical applications in extracting real-world evidence from real-world data.
%

==> content/materials_methods.tex <==
%\section*{Materials and Methods}
%\matmethods{}
